Exploring Interactive Color Palettes for Abstraction-Driven Exploratory Image Colorization

Color design is essential in areas such as product, graphic, and fashion design. However, current tools like Photoshop, with their concrete-driven color manipulation approach, often stumble during early ideation, favoring polished end results over initial exploration. We introduced Mondrian as a test-bed for abstraction-driven approach using interactive color palettes for image colorization. Through a formative study with six design experts, we selected three design options for visual abstractions in color design and developed Mondrian where humans work with abstractions and AI manages the concrete aspects. We carried out a user study to understand the benefits and challenges of each abstraction format and compare the Mondrian with Photoshop. A survey involving 100 participants further examined the influence of each abstraction format on color composition perceptions. Findings suggest that interactive visual abstractions encourage a non-linear exploration workflow and an open mindset during ideation, thus providing better creative affordance.

==> texfiles/1-intro_uist23.tex <==
\section{Introduction}
% \outline{
%  para.1: introduce the ``abstract'' concept; one example of traditional practice; the paradigm after AI comes in, with one HAI example. \\
%  para.2: what we do in this paper (task + target users + solution); what is color design? why color design is important? \\
%  para.3: why color design is challenging: perceptual and operational challenges. \\
%  para.4: what's our solution to overcome the challenges? --- color palette. \\
%  para.5: how our solution solved the two challenges. \\
%  para.6: research questions. \\
%  para.7: summary of what we did in this paper. \\
% }
% Psychological research \cite{welling2007four} has suggested that using representational abstraction can facilitate the exploration of creative possibilities and the solving of insight problems. 
% This is because focusing on the high-level, abstract aspects of an activity, such as the "why" and "what" to do, is more beneficial for receiving inspiration from prior solutions and external resources \cite{root2004artistic, goldschmidt2011avoiding} than thinking about the low-level, concrete aspects of the task, such as the "how" to do it. 
% This approach allows one to consider the overall goals and concepts involved in a task, rather than being bogged down in the specific details, thus better affording creative experimentation \cite{dorta2008design}.

% Abstraction can be a powerful tool for rapid ideation and design futuring \cite{ward2004role}, particularly when used in conjunction with AI \cite{}. 
% By working on abstracted versions of their tasks, practitioners can focus on exploring concepts and high-level ideas, while AI can take these rough, ambiguous ideas and shift them into dynamic design possibilities with concrete details.
% One example of this process is the use of line sketching in TaleBrush \cite{chung2022talebrush}, where users draw rough sketches to guide the narrative without having to write out the entire plot. 
% This allows them to focus on the overall structure and direction of the story, while AI fills and refines details.
% Similarly, Transmogrification \cite{brosz2013transmogrification} supports visualization deformation through user-sketched rough shapes where the sketches serve as an abstraction for the quick visualization shape re-design.
% The scheme of \emph{human work on abstracts, AI works on concretes} emphasizes human agency \cite{} for specifying concept designs while maintaining flexibility and openness to new ideas.
% It is particularly useful in driving design directions, stimulating innovations, and prompting critical discussions.
% \xinyu{Too long, trim to one paragraph.}

% Color design refers to selecting and arranging colors to enhance the aesthetic appeal of a product, space, or visual content, such as graphics or images \cite{}.
% It is essential in various fields, including graphic design, interior design, fashion, and product design.
% As a crucial aspect of visual communication, color design can frame the work's overall mood, tone, and impact on viewers \cite{}.
% \xinyu{@Jian, @Ali, @Ryan: I changed the sequence of the color design paragraph and the psychological research in the abstraction paragraph. I feel this flow might be more clear, want to know your feelings.}
Color design is essential in various fields, including graphics, interior, fashion, and product design.
It refers to selecting and arranging colors to enhance the aesthetic appeal of a product, space, or visual content, such as graphics or images \cite{holtzschue2012understanding}.
As a crucial aspect of visual communication, color design can frame the work's overall mood, tone, and impact on viewers \cite{hummell2006synectics}.
However, achieving a visually appealing color design often requires designers to engage in multiple iterations and experimentations. 
Even those with advanced technical skills in color editing tools often find that the process involves trial and error, which can be quite time-consuming.

% However, coloring graphics or images present both perceptual and operational challenges for designers. 
% It requires a thorough understanding of color theory, color psychology, cultural significance, and the technical skills to apply color in a design \cite{} effectively. 
The challenges for coloring graphics or images can be perceptually and operationally.
In terms of perception, designers tend to base their judgment on the color distribution, combination, and relation, such as the dominant and salient colors \cite{kim2017thoughts} and how they interact with each other \cite{whitfield1990color}. 
However, current image editing tools lack instruments that can effectively reflect such heterogeneous information \cite{kim2017thoughts}, where only a coarse view of color distribution is presented (\eg, histograms). %by providing a broader view of color distribution, such as relative dominance and positions. 
Operationally, current tools either fail to provide fine-grained local color modification tools or force users to focus on too detailed tasks (\eg, region selection).
%current tools often fail to provide precise regional color modification tools or easy-to-use selection tools, leading users to focus on the concrete task of region selection, 
This constrains designers from fully exploring the creative potential of color design.

Psychological research \cite{welling2007four, root2004artistic, goldschmidt2011avoiding} has shown that using \emph{representational abstraction} can greatly facilitate ideation in different design activities; examples include storyboards in film-making \cite{bartindale2012storycrate}, mood board in visual design \cite{lucero2012framing}, and diagrams in architecture planning \cite{clark2012precedents}. 
% \xinyu{@Jian: please check if these examples are proper.}\jian{looks good}
% \jian{add 1-2 short examples}
% For instance, in the film industry, storyboards \cite{} are used early on to conceptualize each scene's essence before committing to a plan, thereby supporting ideation and prompting discussions among filmmakers. \jian{This example is a bit off-topic. Do we have something more related to design? We can delete this sentence and merge it into the previous one.}
% Different abstraction levels, \eg, sketches depicting basic shapes or expressing detailed textures, could enable individuals to focus on different design goals and potentially prompt different inspirations \cite{}. \xinyu{add this sentence because we mention different abstraction levels in RQ1.} \jian{what is the domain of this example abstraction level?} \xinyu{sorry I didn't understand this, please explain more on what do you mean by ``domain''?}
One barrier to abstract thinking is that it requires practitioners to imagine how the abstract will become concrete \cite{paivio1991dual}.
With the integration of AI into creative activities, a new collaboration paradigm has emerged where \emph{humans work on abstracts while AI handles the concretes} \cite{subramonyam2022solving}.
% Such collaboration allows individuals to directly ``see'' the possible concrete versions. \xinyu{trying to make the abstract-AI connection more smooth here (sentences 2, 3, 4, 5).} \jian{this specific sentence ``such...'' can be removed?}
For instance, TaleBrush \cite{chung2022talebrush} allows users to quickly explore different narratives by drawing rough sketches to indicate the fate of the protagonist while AI fills the entire plot. 
Such abstraction-based practices are exceptionally powerful in driving design directions, stimulating innovations, and prompting critical discussions \cite{goldschmidt2006variances}.
% \xinyu{@Jian: I didn't shorten this paragraph currently because I feel clearly explaining the inspirations for ``abstract'' design is important but feel free to correct me if you have different opinions. }\jian{looks okay to me}

Inspired by this, we investigate the feasibility of using color palettes as an interactive abstraction to assist design experts and novices in \emph{color design} ideation with computational colorization techniques. 
% To overcome the above challenges, we propose to exploit color palettes as an interactive abstraction of the image and leverage advanced AI colorization models to accomplish the tedious coloring tasks, following the paradigm of ``humans work on abstracts while AI handles the concretes''.
% We propose exploiting color palettes as an interactive image abstraction coupled with computational colorization models to tackle the above challenges.
Instead of working directly on the image, allowing users to manipulate the color palettes while colorization models automatically apply the palette could provide an intuitive and efficient way to tackle the challenges of color design exploration.
The color palette has historically been used as a static reference for designers to seek inspiration \cite{eckert2000sources}. 
It provides perceptual benefits through different palette formats by depicting the colors of an image in different granular levels, varying from 1D uniform (1D) \cite{itten1970elements}, 1D proportional (1D+)\cite{gijsenijdetermining}, to 2D spatial (2D) format \cite{destijl2023shi}, revealing different aspects of color distribution such as proportion and position in the image (Figure~\ref{fig:palette_demo}). 
% \jian{a small figure here to show an example will be good}
Transforming the palettes from static to interactive brings operational benefits as users can abstractly experiment with different main color combinations while leaving the tedious colorization task to AI models. 
Despite the potential benefits, color palettes have never been investigated as an interactive abstraction of images for facilitating color exploration and reducing operational burden. 
Therefore, we ask two questions: 
\begin{itemize}
    % \item \textbf{RQ1}: how do different formats of color palettes as static abstractions influence human perception towards color compositions?  
    % \item \textbf{RQ2}: how do users interact with different formats of color palettes as interactive abstractions for exploring color designs? and
    \item \textbf{RQ1:} how do users \emph{perceive} and \emph{interact with} different formats of color palettes as interactive abstractions for exploring color designs? and
    \item \textbf{RQ2:} how does the \emph{abstraction-driven} colorization influence users' workflow and creativity compared to the traditional \emph{concretes-based} manipulation?
\end{itemize}

% \xinyu{I am considering to add this RQ3 because RQ2 focuses more on the difference among the three formats while RQ3 emphasizes more on comparison between Mondrian and PhotoShop. Willing to know your opinions.}

% \jian{I feel this paragraph can be removed or moved to a later system design section? I feel we have enough motivation and rationale to study color palettes. Whether it can solve the challenges should be verified in the studies.}
% \xinyu{I feel we still need to mention a little bit, merged it into the previous paragraph.}
% By exploiting color palettes in this manner, the perceptual challenge of color design can be addressed naturally. 
% Color palettes are designed to depict the dominant colors in an image, and different formats reveal different aspects of color distribution, such as proportion or position. 
% Additionally, such interactive palettes together with AI colorization models can also address the operational challenge effectively.
% By transforming the palette from static to interactive, users can focus on exploring different dominant color combinations through the palette, while the AI-powered colorization models automatically apply the color palette to the original image. 
% This allows users to focus on abstract-level ideas and let the AI handle the concrete-level details.


% To answer these questions, we first did a survey study to understand whether different abstraction levels, reflected as various formats of color palettes, influence human perception of color compositions with respect to aesthetic and affective impressions.
% Further, we conducted semi-structured interviews with design novices and experts to understand the current practices and challenges in color design as well as their opinions on taking color palettes as an interactive abstraction in the color design tasks. 
% According to the collected feedback, we developed a system, \sysname{}, incorporating the interactive color palette and AI colorization model to verify the feasibility of using such abstraction for color design ideation.
% Lastly, we carried out an in-lab user study to explore how users interact with color palettes to integrate their intents into the automatic colorization process.
% Through all the studies, we find that employing the abstraction approach---using an interactive color palette as a proxy for colorization---is valued by users for color design exploratory.
% In addition, providing different abstraction levels for users is necessary to suit different design scenarios and accommodate different design stages.

To address these questions, we began by developing the \sysname{}, a system incorporating interactive color palettes and AI colorization models, through an iterative design process with six pilot users. 
This initially validated the feasibility of using abstraction for digital image colorization. 
Subsequently, we conducted an in-lab study to explore users' experiences with different color palettes, as well as how \sysname{} facilitates their creative workflows. 
Feedback from participants highlighted each format offering a unique perspective on color compositions and confirmed the effectiveness of the \emph{abstraction-driven} approach in inspiring diverse design possibilities.
Lastly, we carried out a survey study to systematically and quantitatively assess the impact of different color palette formats on human perception of color compositions. 
Our findings indicate that different palette formats significantly influence the perceived aesthetic quality and affective feelings, contributing valuable insights for future research in this area.
Our contributions are as follows: 
\begin{itemize}
    \item An innovative system that features three distinct formats of interactive color palettes integrated with AI colorization models to facilitate color design exploration and experimentation.
    \item An in-lab user study that offers insights into user perception and interaction with color palettes as interactive abstractions, providing guidance for future research.
    \item A comprehensive survey study that investigates the impact of varying palette formats on human perception of color compositions, revealing their impact on perceived color design aesthetics and affectiveness.
\end{itemize}

\begin{figure}[tb]
    \includegraphics[width=0.98\linewidth]{figures/palette_demo.pdf}
    \vspace{-4mm}
    \caption{Demonstration of 1D uniform (1D) palette, 1D proportional (1D+) palette, and 2D spatial (2D) palette.}
    \label{fig:palette_demo}
    \Description{to fill.}
\end{figure}



